Socially Guided Intrinsic Motivation for Robot Learning of Motor Skills

This paper presents a technical approach to robot learning of motor skills which combines active intrinsically motivated learning with imitation learning. Our architecture, called SGIM-D, allows efficient learning of high-dimensional continuous sensorimotor inverse models in robots, and in particular learns distributions of parameterised motor policies that solve a corresponding distribution of parameterised goals/tasks. This is made possible by the technical integration of imitation learning techniques within an algorithm for learning inverse models that relies on active goal babbling. After reviewing social learning and intrinsic motivation approaches to action learning, we describe the general framework of our algorithm, before detailing its architecture. In an experiment where a robot arm has to learn to use a flexible fishing line , we illustrate that SGIM-D efficiently combines the advantages of social learning and intrinsic motivation and benefits from human demonstration properties to learn how to produce varied outcomes in the environment, while developing more precise control policies in large spaces.

==> Nguyen_bio.tex <==
Sao Mai holds a master degree in computer science from Ecole Polytechnique and a master degree in adaptive machine systems from Osaka University. She started research in cognitive developmental robotics in Asada Lab, Japan, focusing on the theory of mind. She is currently a PhD student in the Flowers Team where she studies how to combine curiosity-driven exploration and socially guided exploration to learn motor skills, focusing on active learning for a strategic student learner to learn several tasks with several strategies, and interactive learning to choose what, who and when to learn from social interaction. Her main topics of interest are developmental robotics, cognitive science, machine learning, imitation learning and intrinsic motivation

==> Oudeyer_bio.tex <==
Dr. Pierre-Yves Oudeyer is permanent researcher at Inria and responsible of the FLOWERS team at Inria and Ensta-ParisTech. Before, he has been a permanent researcher in Sony Computer Science Laboratory for 8 years (1999-2007). He studied theoretical computer science at Ecole Normale SupŽrieure in Lyon, and received his Ph.D. degree in artificial intelligence from the University Paris VI, France. After having worked on computational models of language evolution, he is now working on developmental and social robotics. He has published a book, more than 80 papers in international journals and conferences, holds 8 patents, gave several invited keynote lectures in international conferences, and received several prizes for his work. In particular, he is a laureate of the ERC Starting Grant EXPLORERS. He is editor of the IEEE CIS Newsletter on Autonomous Mental Development, and an associate editor of IEEE Transactions on Autonomous Mental Development, Frontiers in Neurorobotics, and of the International Journal of Social Robotics.

==> Section__Analysis_of_Social_Interaction_Modes.tex <==
\subsection{Analysis of Social Interaction Modes}
**SECTION TO MODIFY**

Within the framework of  learning the forward and the inverse models  of the mapping $ \mathbf{M}: (c, a) \mapsto y$, we would like to introduce the guidance of a human teacher to boost the learning of the means $a$ and goals $y$ in the contexts $c$. Given the model estimated by the robot $M_{R}$, and by the human teacher $M_{H}$, we can consider social interaction as a transformation $SocInter:  (M_R, M_H) \mapsto  (M2_R, M2_H) $.  The social interaction is a combination of these behaviours:
\begin{itemize}
\item the human teacher's behaviour $SocInter_H$ in response to the behaviour of robot and the environment. 
\item the machine learner's behaviour $SocInter_R$ in response to the guidance of the human teacher.
\end{itemize}

The goal of the learning is that the robot acquires a better model of the world in necessary subspaces. 
In order to define the social interaction that we wish to consider, we need to examine the different possibilities and ask ourselves what to imitate, how to imitate, when to imitate and who to imitate \cite{Imitation-and-Social-Learning-in-Robots-Humans-and-Animals:}. The above four questions, which we will address partially in the following section, aim at being generic in the sense of making no assumptions on the type of skills that may be transmitted. 

%
\subsubsection{ Role of the Teacher}
First of all, let us define which type of interaction takes place, and what role we give to the teacher:  

\paragraph{ The teacher provides high-level evaluation to a machine learner}  the teacher would guide the robot through indirect  feedback, or labels such as an estimation of distance between the goal of a specific task and the robot's exploration. This case would meet the more classical frameworks of reinforcement learning or supervised classification.
% \cite{ThomazBreazeal-ConnSci08} used such feedback to boost reinforcement learning. Child development psychology would illustrate the importance of such feedback from teachers to infants for instance by the means of motherese  \cite{springerlink:10.1023/A:1013215010749}. Nevertheless, as in parent-child interaction cheering is completed by games where the parents show and instruct children interesting cases, and help children reach their goal, a more informational interaction would better help the learner than mere cheering.

\paragraph{ The teacher shows how to reach the goal that the robot aims at} the teacher here would show to the robot a means to reach the goal $y_g$ that the robot had set by itself from the given context $c_g$: $SocInter_H(c_g,y_g) \in \{ a \in A | M(c_g, a) = y_g \}$. An applicable case is the example of active learning where the robot asks for demonstrations  \cite{ChernovaVelosoJAIR09} when it makes no progress and does not reach the goal it has set by itself. The robot learns new ways to reach that goal and can replicate the action. This is an imitation behaviour in a restricted definition of the term, where the observer copies the specific motor patterns.

\paragraph{ The teacher shows a context  (new initial conditions)}  $SocInter_H = c \in C$ . The teacher here could set up new situations and contexts, and let the robot learn autonomously in the demonstrated context. This setting would be interesting for a mobile robot that changes location such as exploration, rescue or space robots.

\paragraph{The teacher demonstrates goals} such as in \cite{Cederborg10}, i.e. $SocInter_H = y \in Y $. This would typically help a robot that has been trying to solve tasks of low interest values (the measure of the level of interest depends on the specific experiment). It learns about results and changes that can be accomplished in the environment and attempts to replicate such states and changes. This is the definition of an emulation behaviour, one of the two broad categories of social learning along with imitation \cite{Imitation-in-animals-and-artifacts-chapter-Three-sources-of-information-in-social-learning}. Nevertheless, emulation alone can not satisfyingly represent social learning, as young children are prone to imitate the action sequences, even parts that are not obviously necessary to achieve the goal: a phenomenon known as over-imitation \cite{springerlink:10.1007/s10071-004-0239-6}. 

\paragraph{The teacher shows both a means and a goal} $SocInter_H \in A \times Y $. This is a typical imitation behaviour in the broad sense, where the observer copies both the specific motor patterns and consequent results that are jointly inferred to have been part of the behaviour intention. The new sample  highlights  a subspace  which the robot can explore. This seems to be the most complete approach as it enables both imitation and emulation, as it influences the learner both from the action point of view and the goal point of view.

To sum up, the teacher who shows both a means and a goal seems to offer the best opportunity for the learner to progress, for he provides the learner with both example goals and example means, so that the learner can use both the means and/or the goal-driven approach.


%
\subsubsection{Timing of the Social Interaction}
After these considerations about the nature human teacher's behaviour and guidance $SocInter_H$, our next question is: when should the interaction take place?
 
\paragraph{ In the very beginning} before any personal experience of the robot itself. This would speed up the learning from the beginning, but has no merit as it would not account for the adaptability and flexibility to the changing environment and demand from the user.
\paragraph{ At a regular pace} (every N experiments). This would represent the regular and continuous social interactions the system has with its teacher, and is best to assess quantitatively the improvement of its learning.
\paragraph{ When the robot stops making progress} the measure of progress being specific to the learning problem. Either it asks for help by himself (sends a non null $SocInter_R$ ), or the benevolent teacher steps in. This seems the best solution to maximise the utility of the teacher, but brings questions such as how to evaluate that the robot is stuck, and at which level of difficulty the teacher should step in. It would also assume that the teacher is attentive to the state of the robot.

Although the 3rd case seems interesting theoretically, as the purpose of this work is to compare the performance of different algorithms, we opted for an idealised teacher, who would have continuous interaction with the robot throughout the learning duration. And to make the teaching neutral and not biased to fit our algorithm specifically, we choose non optimal teaching parameters. The teacher gives a demonstration at constant frequency, and randomly selects it from a set of demonstrations.
 
 %
\subsubsection{Which Demonstrations to Choose}
This brings us to the more specific question of which demonstrations among all the possible demonstrations, the teacher should give to the learner:

\paragraph { One sample among a set of completely random examples} this seems the easiest solution but the teaching would not differ from random exploration.
\paragraph { One random among the unreached goals} this solution makes the robot explore new goals and unexplored subspaces.
\paragraph{  The farthest among the unreached goals } it would make sure the new goal provided is not already accessible to the robot, but still, it would prove to be too difficult a goal to help the robot progress.
\paragraph{  The nearest among the unreached goals}  it respects the progressive development idea, but demonstrations would fail to introduce the learner to new unexplored subspaces.

To bootstrap a system endowed with intrinsic motivation, we choose to use a learning by demonstration of means and goals, where the teacher introduces at regular pace a random demonstration among the unreached goals.



